Oblivious Online Monitoring for Safety LTL Specification via Fully Homomorphic Encryption

In many Internet of Things (IoT) applications, data sensed by an IoT device are continuously sent to the server and monitored against a specification. Since the data often contain sensitive information, and the monitored specification is usually proprietary, both must be kept private from the other end. We propose a protocol to conduct oblivious online monitoring -- online monitoring conducted without revealing the private information of each party to the other -- against a safety LTL specification. In our protocol, we first convert a safety LTL formula into a DFA and conduct online monitoring with the DFA. Based on fully homomorphic encryption (FHE), we propose two online algorithms (Reverse and Block) to run a DFA obliviously. We prove the correctness and security of our entire protocol. We also show the scalability of our algorithms theoretically and empirically. Our case study shows that our algorithms are fast enough to monitor blood glucose levels online, demonstrating our protocol's practical relevance.

==> gnuplot-lua-tikz-common.tex <==

\def\gpchecktikzversion#1.#2\relax{%
\ifnum#1<2%
  \errmessage{PGF/TikZ version >= 2.0 is required!}%
\fi}
\expandafter\gpchecktikzversion\pgfversion\relax

\def\gnuplot@output@ps{ps} %

\expandafter\def\csname gnuplot@select@driver@pgfsys-dvi.def\endcsname     {ps}
\expandafter\def\csname gnuplot@select@driver@pgfsys-dvipdfm.def\endcsname {pdf}
\expandafter\def\csname gnuplot@select@driver@pgfsys-dvipdfmx.def\endcsname{pdf}
\expandafter\def\csname gnuplot@select@driver@pgfsys-dvips.def\endcsname   {ps}
\expandafter\def\csname gnuplot@select@driver@pgfsys-pdftex.def\endcsname  {pdf}
\expandafter\def\csname gnuplot@select@driver@pgfsys-luatex.def\endcsname  {pdf}
\expandafter\def\csname gnuplot@select@driver@pgfsys-tex4ht.def\endcsname  {html}
\expandafter\def\csname gnuplot@select@driver@pgfsys-textures.def\endcsname{ps}
\expandafter\def\csname gnuplot@select@driver@pgfsys-vtex.def\endcsname    {ps}
\expandafter\def\csname gnuplot@select@driver@pgfsys-xetex.def\endcsname   {pdf}

\ifcsname gnuplot@select@driver@\pgfsysdriver\endcsname
  \edef\gnuplot@output@mode{\csname gnuplot@select@driver@\pgfsysdriver\endcsname}
\else
  \errmessage{The driver \pgfsysdriver\space is not supported by gnuplot-lua-tikz}%
\fi

\ifcsname PackageWarning\endcsname
  \let\gnuplot@packagewarning\PackageWarning
\else
  \def\gnuplot@packagewarning#1#2{\immediate\write-1{Package #1 Warning: #2}}
\fi


\def\gp@rawimage@pdf#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{/CMYK}%
  \else%
    \def\gp@temp{/RGB}%
  \fi%
  \pgf@sys@bp{#4}\pgfsysprotocol@literalbuffered{0 0}\pgf@sys@bp{#5}%
  \pgfsysprotocol@literalbuffered{0 0 cm}%
  \pgfsysprotocol@literalbuffered{BI /W #2 /H #3 /CS \gp@temp}%
  \pgfsysprotocol@literalbuffered{/BPC 8 /F /AHx ID}%
  \pgfsysprotocol@literal{#6 > EI}%
}
\def\gp@rawimage@ps#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{4}%
  \else%
    \def\gp@temp{3}%
  \fi%
  \pgfsysprotocol@literalbuffered{0 0 translate}%
  \pgf@sys@bp{#4}\pgf@sys@bp{#5}\pgfsysprotocol@literalbuffered{scale}%
  \pgfsysprotocol@literalbuffered{#2 #3 8 [#2 0 0 -#3 0 #3]}%
  \pgfsysprotocol@literalbuffered{currentfile /ASCIIHexDecode filter}%
  \pgfsysprotocol@literalbuffered{false \gp@temp\space colorimage}%
  \pgfsysprotocol@literal{#6 >}%
}
\def\gp@rawimage@html#1#2#3#4#5#6{%
  \gnuplot@packagewarning{gnuplot-lua-tikz}{%
    \noexpand\gp@rawimage is not implemented for \gnuplot@output@mode\space output.%
  }%
}

\expandafter\let\expandafter\gp@rawimage\csname gp@rawimage@\gnuplot@output@mode\endcsname

\def\gploadimage#1#2#3#4#5{%
  \pgftext[left,bottom,x=#1cm,y=#2cm] {\pgfimage[interpolate=false,width=#3cm,height=#4cm]{#5}};%
}

\def\gp@set@size#1{%
  \def\gp@image@size{#1}%
}

\def\gp@rawimage@#1#2#3#4#5#6#7#8{%
  \tikz@scan@one@point\gp@set@size(#6,#7)\relax%
  \tikz@scan@one@point\pgftransformshift(#2,#3)\relax%
  \pgftext{%
    \pgfsys@beginpurepicture%
    \gp@image@size%
    \gp@rawimage{#1}{#4}{#5}{\pgf@x}{\pgf@y}{#8}%
    \pgfsys@endpurepicture%
  }%
}

\def\gprawimage#1#2#3#4#5#6#7#8#9{%
  \ifx&#9&%
    \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}%
  \else
    \ifx\gnuplot@output@mode\gnuplot@output@ps
      \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}%
    \else
      \gploadimage{#2}{#3}{#6}{#7}{#9}%
    \fi
  \fi
}


\def\gnuplottexextension@lua{\string tex}
\def\gnuplottexextension@tikz{\string tex}


\def\gpsetvar#1#2{%
  \expandafter\xdef\csname gp@var@#1\endcsname{#2}
}

\def\gpgetvar#1{%
  \csname gp@var@#1\endcsname %
}


\def\gpfill#1{\path[line width=0.1\gpbaselw,draw,fill,#1]}

\def\gpsetlinewidth#1{\pgfsetlinewidth{#1\gpbaselw}}

\def\gpsetlinetype#1{\tikzset{gp path/.style={#1,#1 add}}}

\def\gpsetdashtype#1{\tikzset{gp path/.append style={#1}}}

\def\gpsetpointsize#1{\tikzset{gp point/.style={mark size=#1\gpbasems}}}

\def\gpcolor#1{\tikzset{global #1}}
\tikzset{rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\tikzset{color=.}}}
\tikzset{global rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\pgfutil@color{.}}}
\tikzset{global color/.code={\pgfutil@color{#1}}}

\newif\ifgpscalepoints
\tikzset{gp shift only/.style={%
  \ifgpscalepoints\else shift only\fi%
}}
\def\gppoint#1#2{%
  \path[solid] plot[only marks,gp point,mark options={gp shift only},#1] coordinates {#2};%
}
\def\gp3point#1#2#3{%
  \path[solid#2] plot[only marks,gp point,mark options={gp shift only},#1] coordinates {#3};%
}


\newdimen\gpvcharsize
\newdimen\gphcharsize
\def\gpcalccharsize{%
  \pgfinterruptboundingbox%
  \pgfsys@begininvisible%
  \node at (0,0) {%
    \global\gphcharsize=1.05\fontcharwd\font`0%
    \global\gpvcharsize=1.05\fontcharht\font`0%
    \global\advance\gpvcharsize by 1.05\fontchardp\font`g%
  };%
  \pgfsys@endinvisible%
  \endpgfinterruptboundingbox%
}

\def\gpdefrectangularnode#1#2#3{%
  \expandafter\gdef\csname pgf@sh@ns@#1\endcsname{rectangle}%
  \expandafter\gdef\csname pgf@sh@np@#1\endcsname{%
    \def\southwest{#2}%
    \def\northeast{#3}%
  }%
  \pgfgettransform\pgf@temp%
  \expandafter\xdef\csname pgf@sh@nt@#1\endcsname{\pgf@temp}%
  \expandafter\xdef\csname pgf@sh@pi@#1\endcsname{\pgfpictureid}%
}



\tikzset{gnuplot/.style={%
  >=stealth',%
  line cap=round,%
  line join=round,%
}}

\tikzset{gp node left/.style={anchor=mid west,yshift=-.12ex,line width=0pt}}
\tikzset{gp node center/.style={anchor=mid,yshift=-.12ex,line width=0pt}}
\tikzset{gp node right/.style={anchor=mid east,yshift=-.12ex,line width=0pt}}

\newdimen\gpbasems
\gpbasems=.4pt

\newdimen\gpbaselw
\gpbaselw=.4pt

\colorlet{gpbgfillcolor}{white}

\def\gpsetbgcolor#1{%
  \pgfutil@definecolor{gpbgfillcolor}{rgb}{#1}%
  \tikzset{tight background,background rectangle/.style={fill=gpbgfillcolor},show background rectangle}%
}

\tikzset{gp refnode/.style={coordinate,yshift=.12ex}}


\def\gpbboxborder{0mm}


\tikzset{gp arrow 1/.style={>=latex}}
\tikzset{gp arrow 2/.style={>=angle 90}}
\tikzset{gp arrow 3/.style={>=angle 60}}
\tikzset{gp arrow 4/.style={>=angle 45}}
\tikzset{gp arrow 5/.style={>=o}}
\tikzset{gp arrow 6/.style={>=*}}
\tikzset{gp arrow 7/.style={>=diamond}}
\tikzset{gp arrow 8/.style={>=open diamond}}
\tikzset{gp arrow 9/.style={>={]}}}
\tikzset{gp arrow 10/.style={>={[}}}
\tikzset{gp arrow 11/.style={>=)}}
\tikzset{gp arrow 12/.style={>=(}}

\tikzset{gp mark 0/.style={mark size=.5\pgflinewidth,mark=*}}
\tikzset{gp mark 1/.style={mark=+}}
\tikzset{gp mark 2/.style={mark=x}}
\tikzset{gp mark 3/.style={mark=star}}
\tikzset{gp mark 4/.style={mark=square}}
\tikzset{gp mark 5/.style={mark=square*}}
\tikzset{gp mark 6/.style={mark=o}}
\tikzset{gp mark 7/.style={mark=*}}
\tikzset{gp mark 8/.style={mark=triangle}}
\tikzset{gp mark 9/.style={mark=triangle*}}
\tikzset{gp mark 10/.style={mark=triangle,every mark/.append style={rotate=180}}}
\tikzset{gp mark 11/.style={mark=triangle*,every mark/.append style={rotate=180}}}
\tikzset{gp mark 12/.style={mark=diamond}}
\tikzset{gp mark 13/.style={mark=diamond*}}
\tikzset{gp mark 14/.style={mark=otimes}}
\tikzset{gp mark 15/.style={mark=oplus}}

\tikzset{gp pattern 0/.style={white}}
\tikzset{gp pattern 1/.style={pattern=north east lines}}
\tikzset{gp pattern 2/.style={pattern=north west lines}}
\tikzset{gp pattern 3/.style={pattern=crosshatch}}
\tikzset{gp pattern 4/.style={pattern=grid}}
\tikzset{gp pattern 5/.style={pattern=vertical lines}}
\tikzset{gp pattern 6/.style={pattern=horizontal lines}}
\tikzset{gp pattern 7/.style={pattern=dots}}
\tikzset{gp pattern 8/.style={pattern=crosshatch dots}}
\tikzset{gp pattern 9/.style={pattern=fivepointed stars}}
\tikzset{gp pattern 10/.style={pattern=sixpointed stars}}
\tikzset{gp pattern 11/.style={pattern=bricks}}

\tikzset{gp plot axes/.style=}
\tikzset{gp plot border/.style=}
\tikzset{gp plot 0/.style=smooth}
\tikzset{gp plot 1/.style=smooth}
\tikzset{gp plot 2/.style=smooth}
\tikzset{gp plot 3/.style=smooth}
\tikzset{gp plot 4/.style=smooth}
\tikzset{gp plot 5/.style=smooth}
\tikzset{gp plot 6/.style=smooth}
\tikzset{gp plot 7/.style=smooth}

\tikzset{gp lt axes/.style=dotted}
\tikzset{gp lt border/.style=solid}

\tikzset{gp lt axes add/.style={}}
\tikzset{gp lt border add/.style={}}
\tikzset{gp lt plot 0 add/.style={}}
\tikzset{gp lt plot 1 add/.style={}}
\tikzset{gp lt plot 2 add/.style={}}
\tikzset{gp lt plot 3 add/.style={}}
\tikzset{gp lt plot 4 add/.style={}}
\tikzset{gp lt plot 5 add/.style={}}
\tikzset{gp lt plot 6 add/.style={}}
\tikzset{gp lt plot 7 add/.style={}}
\tikzset{gp lt plot 0/.style={}}
\tikzset{gp lt plot 1/.style={}}
\tikzset{gp lt plot 2/.style={}}
\tikzset{gp lt plot 3/.style={}}
\tikzset{gp lt plot 4/.style={}}
\tikzset{gp lt plot 5/.style={}}
\tikzset{gp lt plot 6/.style={}}
\tikzset{gp lt plot 7/.style={}}

\colorlet{gp lt color axes}{black!30}
\colorlet{gp lt color border}{black}

\def\gpdashlength{\pgflinewidth}
\tikzset{gp dt 0/.style={solid}}
\tikzset{gp dt 1/.style={solid}}
\tikzset{gp dt 2/.style={dash pattern=on 7.5*\gpdashlength off 7.5*\gpdashlength}}
\tikzset{gp dt 3/.style={dash pattern=on 3.75*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 4/.style={dash pattern=on 1*\gpdashlength off 2.8125*\gpdashlength}}
\tikzset{gp dt 5/.style={dash pattern=on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt 6/.style={dash pattern=on 5.625*\gpdashlength off 5.625*\gpdashlength on 1*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 7/.style={dash pattern=on 3.75*\gpdashlength off 3.75*\gpdashlength on 3.75*\gpdashlength off 11.25*\gpdashlength}}
\tikzset{gp dt 8/.style={dash pattern=on 1*\gpdashlength off 3.75*\gpdashlength on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt solid/.style={solid}}
\tikzset{gp dt axes/.style={dotted}}

\def\gpcoloredlines{%
  \colorlet{gp lt color 0}{red}%
  \colorlet{gp lt color 1}{green}%
  \colorlet{gp lt color 2}{blue}%
  \colorlet{gp lt color 3}{magenta}%
  \colorlet{gp lt color 4}{cyan}%
  \colorlet{gp lt color 5}{yellow}%
  \colorlet{gp lt color 6}{orange}%
  \colorlet{gp lt color 7}{purple}%
}

\def\gpmonochromelines{%
  \colorlet{gp lt color 0}{black}%
  \colorlet{gp lt color 1}{black}%
  \colorlet{gp lt color 2}{black}%
  \colorlet{gp lt color 3}{black}%
  \colorlet{gp lt color 4}{black}%
  \colorlet{gp lt color 5}{black}%
  \colorlet{gp lt color 6}{black}%
  \colorlet{gp lt color 7}{black}%
}

\gpcoloredlines
\gpsetpointsize{4}
\gpsetlinetype{gp lt solid}
\gpscalepointsfalse
\endinput


==> gnuplot-lua-tikz.tex <==
\input tikz.tex
\usetikzlibrary{arrows,patterns,plotmarks,backgrounds,fit}

\edef\tikzatcode{\the\catcode`\@}
\catcode`\@=11

\input gnuplot-lua-tikz-common.tex

\catcode`\@=\tikzatcode

\endinput


==> m20211231-fixed-input.tex <==
\begin{tikzpicture}[gnuplot]
\path (0.000,0.000) rectangle (6.000,3.100);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.320,0.985)--(1.500,0.985);
\draw[gp path] (5.447,0.985)--(5.267,0.985);
\node[gp node right] at (1.136,0.985) {$0$};
\draw[gp path] (1.320,1.437)--(1.500,1.437);
\draw[gp path] (5.447,1.437)--(5.267,1.437);
\node[gp node right] at (1.136,1.437) {$50$};
\draw[gp path] (1.320,1.888)--(1.500,1.888);
\draw[gp path] (5.447,1.888)--(5.267,1.888);
\node[gp node right] at (1.136,1.888) {$100$};
\draw[gp path] (1.320,2.340)--(1.500,2.340);
\draw[gp path] (5.447,2.340)--(5.267,2.340);
\node[gp node right] at (1.136,2.340) {$150$};
\draw[gp path] (1.320,2.791)--(1.500,2.791);
\draw[gp path] (5.447,2.791)--(5.267,2.791);
\node[gp node right] at (1.136,2.791) {$200$};
\draw[gp path] (1.320,0.985)--(1.320,1.165);
\draw[gp path] (1.320,2.791)--(1.320,2.611);
\node[gp node center] at (1.320,0.677) {$0$};
\draw[gp path] (2.129,0.985)--(2.129,1.165);
\draw[gp path] (2.129,2.791)--(2.129,2.611);
\node[gp node center] at (2.129,0.677) {$100$};
\draw[gp path] (2.938,0.985)--(2.938,1.165);
\draw[gp path] (2.938,2.791)--(2.938,2.611);
\node[gp node center] at (2.938,0.677) {$200$};
\draw[gp path] (3.748,0.985)--(3.748,1.165);
\draw[gp path] (3.748,2.791)--(3.748,2.611);
\node[gp node center] at (3.748,0.677) {$300$};
\draw[gp path] (4.557,0.985)--(4.557,1.165);
\draw[gp path] (4.557,2.791)--(4.557,2.611);
\node[gp node center] at (4.557,0.677) {$400$};
\draw[gp path] (5.366,0.985)--(5.366,1.165);
\draw[gp path] (5.366,2.791)--(5.366,2.611);
\node[gp node center] at (5.366,0.677) {$500$};
\draw[gp path] (1.320,2.791)--(1.320,0.985)--(5.447,0.985)--(5.447,2.791)--cycle;
\node[gp node center,rotate=-270] at (0.292,1.888) {time (sec)};
\node[gp node center] at (3.383,0.215) {\# of States (states)};
\node[gp node right] at (3.979,2.457) {\ReverseStream{}};
\gpsetlinewidth{2.00}
\draw[gp path] (4.163,2.457)--(5.079,2.457);
\draw[gp path] (1.401,1.082)--(1.725,1.126)--(2.129,1.146)--(2.938,1.187)--(3.748,1.232)%
  --(4.557,1.269)--(5.366,1.313);
\gpsetpointsize{4.00}
\gp3point{gp mark 1}{}{(1.401,1.082)}
\gp3point{gp mark 1}{}{(1.725,1.126)}
\gp3point{gp mark 1}{}{(2.129,1.146)}
\gp3point{gp mark 1}{}{(2.938,1.187)}
\gp3point{gp mark 1}{}{(3.748,1.232)}
\gp3point{gp mark 1}{}{(4.557,1.269)}
\gp3point{gp mark 1}{}{(5.366,1.313)}
\gp3point{gp mark 1}{}{(4.621,2.457)}
\node[gp node right] at (3.979,2.149) {\BlockStream{}};
\gpsetdashtype{gp dt 2}
\draw[gp path] (4.163,2.149)--(5.079,2.149);
\draw[gp path] (1.401,1.661)--(1.725,1.697)--(2.129,1.798)--(2.938,1.868)--(3.748,1.956)%
  --(4.557,2.004)--(5.366,2.055);
\gp3point{gp mark 2}{}{(1.401,1.661)}
\gp3point{gp mark 2}{}{(1.725,1.697)}
\gp3point{gp mark 2}{}{(2.129,1.798)}
\gp3point{gp mark 2}{}{(2.938,1.868)}
\gp3point{gp mark 2}{}{(3.748,1.956)}
\gp3point{gp mark 2}{}{(4.557,2.004)}
\gp3point{gp mark 2}{}{(5.366,2.055)}
\gp3point{gp mark 2}{}{(4.621,2.149)}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.320,2.791)--(1.320,0.985)--(5.447,0.985)--(5.447,2.791)--cycle;
\gpdefrectangularnode{gp plot 1}{\pgfpoint{1.320cm}{0.985cm}}{\pgfpoint{5.447cm}{2.791cm}}
\end{tikzpicture}


==> m20211231-fixed-state.tex <==
\begin{tikzpicture}[gnuplot]
\path (0.000,0.000) rectangle (6.000,3.100);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.320,0.985)--(1.500,0.985);
\draw[gp path] (5.447,0.985)--(5.267,0.985);
\node[gp node right] at (1.136,0.985) {$0$};
\draw[gp path] (1.320,1.437)--(1.500,1.437);
\draw[gp path] (5.447,1.437)--(5.267,1.437);
\node[gp node right] at (1.136,1.437) {$50$};
\draw[gp path] (1.320,1.888)--(1.500,1.888);
\draw[gp path] (5.447,1.888)--(5.267,1.888);
\node[gp node right] at (1.136,1.888) {$100$};
\draw[gp path] (1.320,2.340)--(1.500,2.340);
\draw[gp path] (5.447,2.340)--(5.267,2.340);
\node[gp node right] at (1.136,2.340) {$150$};
\draw[gp path] (1.320,2.791)--(1.500,2.791);
\draw[gp path] (5.447,2.791)--(5.267,2.791);
\node[gp node right] at (1.136,2.791) {$200$};
\draw[gp path] (1.725,0.985)--(1.725,1.165);
\draw[gp path] (1.725,2.791)--(1.725,2.611);
\node[gp node center] at (1.725,0.677) {$10$};
\draw[gp path] (2.534,0.985)--(2.534,1.165);
\draw[gp path] (2.534,2.791)--(2.534,2.611);
\node[gp node center] at (2.534,0.677) {$20$};
\draw[gp path] (3.343,0.985)--(3.343,1.165);
\draw[gp path] (3.343,2.791)--(3.343,2.611);
\node[gp node center] at (3.343,0.677) {$30$};
\draw[gp path] (4.152,0.985)--(4.152,1.165);
\draw[gp path] (4.152,2.791)--(4.152,2.611);
\node[gp node center] at (4.152,0.677) {$40$};
\draw[gp path] (4.961,0.985)--(4.961,1.165);
\draw[gp path] (4.961,2.791)--(4.961,2.611);
\node[gp node center] at (4.961,0.677) {$50$};
\draw[gp path] (1.320,2.791)--(1.320,0.985)--(5.447,0.985)--(5.447,2.791)--cycle;
\node[gp node center,rotate=-270] at (0.292,1.888) {time (sec)};
\node[gp node center] at (3.383,0.215) {\# of Monitored Ciphertexts ($\times 10^3$)};
\node[gp node right] at (3.979,2.457) {\ReverseStream{}};
\gpsetlinewidth{2.00}
\draw[gp path] (4.163,2.457)--(5.079,2.457);
\draw[gp path] (1.725,1.049)--(2.534,1.114)--(3.343,1.184)--(4.152,1.248)--(4.961,1.313);
\gpsetpointsize{4.00}
\gp3point{gp mark 1}{}{(1.725,1.049)}
\gp3point{gp mark 1}{}{(2.534,1.114)}
\gp3point{gp mark 1}{}{(3.343,1.184)}
\gp3point{gp mark 1}{}{(4.152,1.248)}
\gp3point{gp mark 1}{}{(4.961,1.313)}
\gp3point{gp mark 1}{}{(4.621,2.457)}
\node[gp node right] at (3.979,2.149) {\BlockStream{}};
\gpsetdashtype{gp dt 2}
\draw[gp path] (4.163,2.149)--(5.079,2.149);
\draw[gp path] (1.725,1.206)--(2.534,1.425)--(3.343,1.642)--(4.152,1.845)--(4.961,2.055);
\gp3point{gp mark 2}{}{(1.725,1.206)}
\gp3point{gp mark 2}{}{(2.534,1.425)}
\gp3point{gp mark 2}{}{(3.343,1.642)}
\gp3point{gp mark 2}{}{(4.152,1.845)}
\gp3point{gp mark 2}{}{(4.961,2.055)}
\gp3point{gp mark 2}{}{(4.621,2.149)}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.320,2.791)--(1.320,0.985)--(5.447,0.985)--(5.447,2.791)--cycle;
\gpdefrectangularnode{gp plot 1}{\pgfpoint{1.320cm}{0.985cm}}{\pgfpoint{5.447cm}{2.791cm}}
\end{tikzpicture}


==> t-gnuplot-lua-tikz.tex <==
\usemodule[tikz]

\usetikzlibrary[arrows,patterns,plotmarks,backgrounds,fit]

\edef\tikzatcode{\the\catcode`\@}
\edef\tikzbarcode{\the\catcode`\|}
\edef\tikzexclaimcode{\the\catcode`\!}
\catcode`\@=11
\catcode`\|=12
\catcode`\!=12

\input gnuplot-lua-tikz-common.tex

\catcode`\@=\tikzatcode
\catcode`\|=\tikzbarcode
\catcode`\!=\tikzexclaimcode

\endinput

